ALIGN: Aligning Condition Estimation and Expression in Advantage-Conditioned Behavior Cloning

Human-collected robot manipulation data often mix successful behavior with retries, pauses, recoveries, and failures. Advantage-Conditioned Behavior Cloning (AC-BC) can exploit such mixed-quality data, but only if the conditioning signal is both accurately constructed from offline trajectories and effectively incorporated into the policy's action-vector-field prediction. Existing pipelines can weaken this signal by thresholding estimator-derived advantage scores into noisy conditions, and by routing conditions through prompts that weakly affect the action vector field. We introduce ALIGN, a condition-aligned AC-BC framework for vision-language-action policies. ALIGN directly predicts categorical pairwise conditions in the policy-facing label space and injects them into a DiT action expert through AdaRMS modulation fused with flow time. We evaluate ALIGN on deliberately mixed real-robot datasets for ARX X5 bowl stacking and Franka key hanging, each combining standard demonstrations with retry-heavy trajectories. ALIGN improves condition fidelity, strengthens conditional vector-field separability, and achieves 90.0% and 56.7% closed-loop success, compared with 56.7% and 33.3% for the strongest AC-BC baseline. These results indicate that aligning conditions from estimation to action prediction is an effective way to extract robust manipulation policies from data in which success, recovery and error coexist.

==> sections/03_preliminaries.tex <==
\section{Preliminaries}

==> tables/table2_policy_results.tex <==
\begin{table}[htbp]
  \centering
  \small
  \caption{Closed-loop policy success over 30 rollouts per variant on ARX X5 bowl stacking and Franka key hanging. The upper block compares condition construction under prompt/default injection; the lower block fixes the direct binary estimator and compares condition-injection mechanisms.}
  \label{tab:policy_eval}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}lllcc@{}}
    \toprule
    Policy variant & Condition source & Injection & ARX X5 bowl stacking & Franka key hanging \\
    \midrule
    \rowcolor{gray!8}
    \multicolumn{5}{@{}l}{\textit{Condition construction comparison}} \\
    SFT, 100 demonstrations & none & none & 46.7\% & 6.7\% \\
    SFT, 100 demonstrations + 100 retry trajectories & none & none & 50.0\% & 3.3\% \\
    \(\pi^*_{0.6}\)-style threshold & continuous progress & prompt/default & 50.0\% & 26.7\% \\
    \(\chi_0\)-style threshold & continuous progress & prompt/default & 56.7\% & 33.3\% \\
    2-class direct estimator & binary categorical & prompt & \textbf{70.0\%} & \textbf{40.0\%} \\
    3-class direct estimator & tri-class categorical & prompt & 66.7\% & 20.0\% \\
    \midrule
    \rowcolor{gray!8}
    \multicolumn{5}{@{}l}{\textit{Condition injection comparison with the direct binary estimator}} \\
    2-class direct estimator & binary categorical & prompt & 70.0\% & 40.0\% \\
    2-class direct estimator & binary categorical & embedding addition & 76.7\% & 40.0\% \\
    2-class direct estimator & binary categorical & per-layer additive & 83.3\% & 40.0\% \\
    2-class direct estimator & binary categorical & outcome token & 76.7\% & 53.3\% \\
    \rowcolor{gray!18}
    ALIGN & binary categorical & AdaRMS & \textbf{90.0\%} & \textbf{56.7\%} \\
    \midrule
    \rowcolor{gray!8}
    \multicolumn{5}{@{}l}{\textit{Additional label-space variant}} \\
    3-class direct estimator & tri-class categorical & AdaRMS & 86.7\% & 33.3\% \\
    \bottomrule
  \end{tabular}%
  }
\end{table}

